Circuit and System Technologies for Energy-Efficient Edge Robotics

As we march towards the age of ubiquitous intelligence, we note that AI and intelligence are progressively moving from the cloud to the edge. The success of Edge-AI is pivoted on innovative circuits and hardware that can enable inference and limited learning in resource-constrained edge autonomous systems. This paper introduces a series of ultra-low-power accelerator and system designs on enabling the intelligence in edge robotic platforms, including reinforcement learning neuromorphic control, swarm intelligence, and simultaneous mapping and localization. We put an emphasis on the impact of the mixed-signal circuit, neuro-inspired computing system, benchmarking and software infrastructure, as well as algorithm-hardware co-design to realize the most energy-efficient Edge-AI ASICs for the next-generation intelligent and autonomous systems.

==> tabs/slam.tex <==
\begin{table}[t!]
\caption{Comparison of different SLAM algorithms.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
                                                                                  & \begin{tabular}[c]{@{}c@{}}\textbf{Probabilistic}\\ \textbf{SLAM}  \end{tabular}                                & \begin{tabular}[c]{@{}c@{}}\textbf{Keyframe-based}\\ \textbf{SLAM}  \end{tabular}                            & \textbf{NeuroSLAM}                                                                                               \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Algorithm of \\ data association\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Direct method, \\ feature-based method \\ (SIFT, SURF, CNN, etc.)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Direct method with maxpooled \\ images \& SNN-based \\ pose-cell activities\end{tabular} \\ \hline
\textbf{Sensor}                                                                   & \multicolumn{2}{c|}{Monocular, stereo, RGB-D camera, etc.}                                                                   & Monocular camera                                                                                                 \\ \hline
\textbf{Odometry}                                                                 & \multicolumn{2}{c|}{Visual odometry, inertia sensor}                                                                         & Visual odometry                                                                                                  \\ \hline
\textbf{Map maintenance}                                                          & Every frame                                                  & Keyframe                                                      & VT-matched frame                                                                                                 \\ \hline
\textbf{Application}                                                              & \multicolumn{2}{c|}{High-performance AR, VR, UAVs}                                                                           & Ultra low power microrobotics                                                                                    \\ \hline
\end{tabular}
\label{tab:slam}
}
% \vspace{-5pt}
\end{table}
